Shrewd Selection Speeds Surfing: Use Smart EXP3!

In this paper, we explore the use of multi-armed bandit online learning techniques to solve distributed resource selection problems. As an example, we focus on the problem of network selection. Mobile devices often have several wireless networks at their disposal. While choosing the right network is vital for good performance, a decentralized solution remains a challenge. The impressive theoretical properties of multi-armed bandit algorithms, like EXP3, suggest that it should work well for this type of problem. Yet, its real-word performance lags far behind. The main reasons are the hidden cost of switching networks and its slow rate of convergence. We propose Smart EXP3, a novel bandit-style algorithm that (a) retains the good theoretical properties of EXP3, (b) bounds the number of switches, and (c) yields significantly better performance in practice. We evaluate Smart EXP3 using simulations, controlled experiments, and real-world experiments. Results show that it stabilizes at the optimal state, achieves fairness among devices and gracefully deals with transient behaviors. In real world experiments, it can achieve 18% faster download over alternate strategies. We conclude that multi-armed bandit algorithms can play an important role in distributed resource selection problems, when practical concerns, such as switching costs and convergence time, are addressed.

==> algorithm/chooseGreedy.tex <==
\begin{algorithm}[!htb]
  \DontPrintSemicolon % so semicolon is not appended at end of \lif
  \Input{$p$, real $y \in (0, 1]$, $l_{i_+}$ $l_{greedy} \in \mathbb{Z}$}
  \Output{$True$ if selection must be greedy and $False$ otherwise}
  \BlankLine 
  \If{$((max(p) - min(p)) \le y$ OR $l_{i_+} \leq l_{greedy})$} 
  {coinFlip $\leftarrow$ outcome of flipping an unbiased coin \\
  \lIf{$coinFlip = Head$} {return True}
  \lElse{return False}
  }
  \lElse{return False}
  \caption{chooseGreedily: determines whether greedy selection must be made}
  \label{algorithm:chooseGreedy}
\end{algorithm}

==> algorithm/networkQualityDecline.tex <==
\begin{algorithm}[!htb]
  \DontPrintSemicolon % so semicolon is not appended at end of \lif
  \Input{$t_{i_+}$, $t_{reset}$, $h_{i_{max}}$, rolling average window size $s$, \% drop considered significant $drop$}
  \Output{$True$ if $i_{max}$ has been selected for $\ge t_{reset}$ consecutive time slots and its quality has dropped significantly, and $False$ otherwise}
  \BlankLine
  \If{size($h_{i_{max}}$) $ \le s$ OR $t_{i_+} < t_{reset}$}{return False}
  $h \leftarrow $ rolling mean of $h_{i_{max}}$ over $s$ gains \\
  $\Delta gain \leftarrow$ change in gain of $i_{max}$, based on $h$\\
  \If{$(\Delta gain < 0)$ AND $(abs(\Delta gain) \ge \frac{(drop\ *\ h_0}{100})$}{return True}{return False}
  \caption{networkQualityDecline: determines if there is a need for reset due to significant decline in the quality of network $i_{max}$}
  \label{algorithm:networkQualityDecline}
\end{algorithm}

==> algorithm/periodicReset.tex <==
\begin{algorithm}[!htb]
  \DontPrintSemicolon % so semicolon is not appended at end of \lif
  \Input{$p_{i_+}, l_{i_+}, p_{high} \in (0,1), l_{reset} \in \mathbb{Z}$}
  \Output{$True$ if a periodic reset is required and $False$ otherwise}
  \BlankLine 
  \lIf{$p_{i_+} \ge p_{high}$ AND $l_{i_+} \ge l_{reset}$}{return $True$}
  \lElse{return $False$}
  \caption{periodicReset: determines whether a periodic reset is required.}
  \label{algorithm:periodicReset}
\end{algorithm}

==> algorithm/reset.tex <==
\begin{algorithm}[!htb]
  \DontPrintSemicolon % so semicolon is not appended at end of \lif
  \Input{$available\_network$}
  \BlankLine 
  ${x}_{i} \leftarrow 0$ for $ i = 1, \cdots, K $  \\reset per network details used for greedy choice
  \\reset monitoring details of $i_{max}$
  \\$explore\_network \leftarrow available\_network$ \\
  start a new block $b$ \\ 
  \caption{reset: performs a reset of the algorithm}
  \label{algorithm:reset}
\end{algorithm}

==> algorithm/switchBack.tex <==
\begin{algorithm}[!htb]
  \DontPrintSemicolon % so semicolon is not appended at end of \lif
  \Input{$i_{b}$, $i_{b-1}$, $available\_network$, $g_{i_b}(t-1)$, last \textit{z} elements of $h_{i_{b-1}}$}
  \Output{$True$ if quality of current network is worse than that of previous and $False$ otherwise}
  \BlankLine 
  \If{switch back in $(b - 1) = False$ AND $i_b \neq i_{b - 1}$ AND $i_{(b - 1)} \in available\_network$) AND $\sum\limits_{a=1}^z (h{i_{b-1}}(a)) > 0$ AND $(g_{i_b}(t-1) < \frac{1}{z} \sum\limits_{a=1}^z h_{i_{b-1}}(a)$ OR $g_{i_b}(t-1) < h_{i_{b-1}}(z)$ OR $(\frac{100}{z} \sum\limits_{a=1}^z (h{i_{b-1}}(a)) > g_{i_b}(t-1)) > 50)$}{return $True$}
  \lElse{return $False$}
  \caption{mustSwitchBack: identifies whether the quality of the wireless network to which a device is connected is worse than the one to which it was connected in the previous block, hence requiring a switch back}
  \label{algorithm:switchBack}
\end{algorithm}

==> algorithm/updateAvailableNetwork.tex <==
\begin{algorithm}[!htb]
  \DontPrintSemicolon % so semicolon is not appended at end of \lif
  \Input{$available\_network$, $lost\_network$, $new\_network$, $i(t-1)$, $w$, $i_+$, $p_{i_+}$, $p_{high}$}
  \BlankLine
  \lIf{($p_{i_+} \geq p_{high}$ AND $i_+ \notin available\_network$) OR new\_network $\neq \O$}{reset()}
  \ElseIf{$i(t-1) \notin available\_network$}{start a new block $b$}
  \ForEach{network $i \in lost\_network$}{
     {delete details pertaining to $i$}
    }
  \Comment{at this point $w$ includes weights of networks still available}
  \lIf{$size(w) \neq 0$}{${w}_{max} \leftarrow max(w)$}
  \lElse{${w}_{max} \leftarrow 1$}
  \lForEach{network $ i \in new\_network$}{
     {$w_i \leftarrow w_{max}$}
     }
     % to explore newly discovered networks with high probability
%   $available\_network \leftarrow (available\_network \backslash lost\_network) \cup new\_network$ \\
  \caption{updateAvailableNetwork: update made when there is a change in the set of networks available}
  \label{algorithm:updateAvailableNetwork}
\end{algorithm}

% other parameters not listed explicitly as they are not explicitly given in the pseudocode of stable hybrid block EXP3 either
% normalization of weights not specified

 %The set difference A\B is defined by
%A\B={x:x in A and x not in B}. 

==> evaluation.tex <==
% This section show that EXP3 has poor practical performance in a dynamic wireless network setting. The performance of Smart EXP3 is evaluated, through simulation and experiments, with respect to the requirements defined in section \ref{subsection:goals}. Each device performs an independent selection, without any  additional overhead on the networks and without the need for any change to the existing network infrastructure.  

This section shows that EXP3 has poor performance in a dynamic wireless network setting. It then evaluates Smart EXP3, relying on artificial simulations (Section \ref{section:evaluationSimulation}), trace-driven simulations (Section \ref{section:evaluationSimulationNetworkTrace}), controlled experiments (Section \ref{section:evaluationExperimentControlled}), and experiments in the wild (Section \ref{section:evaluationExperimentWild}).

\noindent\textbf{Parameter choice.} In our implementation, $\gamma = t^{\frac{-1}{3}}$\cite{maghsudi2013relay}, which tends to zero to ensure convergence \cite{tekin2011performance}; $\beta = 0.1$ such that blocks are short during exploration; and the duration of one time slot is 15 seconds. Smart EXP3 selects greedily with probability $\frac{1}{2}$ when: (1) $max(p)-min(p)\le\frac{1}{K-1}$ or (2) $l_{i_+} < y$, where $y$ is the value of $l_{i_+}$ when $max(p)-min(p)>\frac{1}{K-1}$ for the first time. %Based on empirical results, these are good choices. 
To ignore stale data, a \enquote{switch back} decision is based on observations from only the last 8 time slots of the previous block. The algorithm resets when $p_{i_+} \ge 0.75$ and $l_{i_+} \ge 40$, or a drop of at least 15\% is observed in $i_{max}$ to which the device is connected for more than 4 time slots. This allows fast adaptation while preventing frequent resets.%, without being over-sensitive. 

% table~\ref{table:parameterValues}.
% \input{table/algorithm_parameterValues}
\subsection{Simulation} \label{section:evaluationSimulation}
    \input{evaluation_simulations}
\subsection{Trace-driven simulation} \label{section:evaluationSimulationNetworkTrace}
    \input{evaluation_simulation_network_trace}
\subsection{Controlled experiments}\label{section:evaluationExperimentControlled}
    \input{evaluation_experiment_controlled}
\subsection{Experiments in the wild}\label{section:evaluationExperimentWild}
    \input{evaluation_experiment_wild}

==> table/algorithm_parameterValues.tex <==
\begin{table}[!htb]
\caption{Parameter values.}
\label{table:parameterValues}
\centering 
\begin{tabularx}\linewidth{|c|c|X|}
\hline
Parameter & Value & Justification \\
\hline
$\gamma$ & $t^{\frac{-1}{3}}$ & Tends to zero, as required for convergence, also used in \cite{maghsudi2013relay}] \\
\hline
$\beta$ & $0.1$ & Block lengths are small during initial exploration. \\
\hline
$y$ & $\frac{1}{k - 1} $ & Seems a good choice based on empirical results. \\
\hline
% $l_{greedy}$ & \multicolumn{2}{|l|}{Set to block length of $i_+$ when $(max(p) - min(p)) > y$} \\
$l_{greedy}$ & Min of 2 & $l_{i_+}$ when (max(p) - min(p)) $>$ y gives good result. \\
\hline
$z$ & $8$ & Ignores stale observations in a highly dynamic setting. \\
\hline
$p_{high}$ & $0.75$ & Allow fast adaptation while preventing frequent resets. \\
\hline
$l_{reset}$ & $40$ & Allow fast adaptation while preventing frequent resets. \\
\hline
$t_{reset}$ & $4$ & Allows Smart EXP3 to react quickly to changes. \\
\hline
$drop$ & $15$ & Allows fast adaptation without being too sensitive. \\
\hline
$s$ & $12$ & Ignores noise in observations, based on empirical results. \\
\hline
% $\eta$ & & $\sqrt{\frac{8\ ln(K)}{t}}$\\
% \hline
\end{tabularx}
\end{table}

==> table/cumulativeGain_simulation.tex <==
\begin{table}[!htb]
\small
\centering
\caption{Per client cumulative gain --- median (MB) and standard deviation (MB).}
\label{table:static_rateOfConvergence}
\begin{tabular}{lcccc}
% \cline{2-4}
\hline
\textbf{}                              & \multicolumn{2}{c}{\textbf{Setting 1}} & \multicolumn{2}{c}{\textbf{Setting 2}}   \\ %\cline{2-4} 
\textbf{} & \textbf{Median (MB)} & \textbf{std (MB)} & \textbf{Median (MB)} & \textbf{std (MB)} \\ \hline
% \multicolumn{1}{l}{\textbf{EXP3}} & 2889.77 & 134.14 & 2731.04 & 84.31 \\
% \hline
% \multicolumn{1}{l}{\textbf{Block EXP3}}  & 3531.10 & 506.49 & 3572.38 & 424.17 \\
% \hline
% \multicolumn{1}{l}{\textbf{Hybrid Block EXP3}}  & 3486.45 & 668.62 & 3551.42 & 250.01 \\
% \hline
% \multicolumn{1}{l}{\textbf{Smart EXP3 w/o reset}} & 3526.06 & 267.58 & 3543.97 & 217.67 \\
% \hline
% \multicolumn{1}{l}{\textbf{Smart EXP3}} & 3530.99 & 194.25 & 3618.66 & 94.18 \\
% \hline
% \multicolumn{1}{l}{\textbf{Greedy}} & 3141.58 & 618.17 & 3534.67 & 599.36 \\
% \hline
% \multicolumn{1}{l}{\textbf{Full information}} & 2920.22 & 55.53 & 2704.38 & 92.53 \\
% \hline
% \multicolumn{1}{l}{\textbf{Centralized}} & 3534.59 & 306.51 & 3534.58 & 269.96 \\
% \hline
% \multicolumn{1}{l}{\textbf{Fixed random}} & 2249.17 & 3319.02 & 3534.33 & 1365.35 \\
% \hline
\multicolumn{1}{l}{\textbf{EXP3}} & 2.89 & 0.13 & 2.73 & 0.08 \\
\hline
\multicolumn{1}{l}{\textbf{Block EXP3}}  & 3.53 & 0.51 & 3.57 & 0.42 \\
\hline
\multicolumn{1}{l}{\textbf{Hybrid Block EXP3}}  & 3.49 & 0.67 & 3.55 & 0.25 \\
\hline
\multicolumn{1}{l}{\textbf{Smart EXP3 w/o Reset}} & 3.53 & 0.27 & 3.54 & 0.22 \\
\hline
\multicolumn{1}{l}{\textbf{Smart EXP3}} & 3.53 & 0.19 & 3.62 & 0.09 \\
\hline
\multicolumn{1}{l}{\textbf{Greedy}} & 3.14 & 0.62 & 3.53 & 0.60 \\
\hline
\multicolumn{1}{l}{\textbf{Full Information}} & 2.92 & 0.06 & 2.70 & 0.09 \\
\hline
\multicolumn{1}{l}{\textbf{Centralized}} & 3.53 & 0.31 & 3.53 & 0.27 \\
\hline
\multicolumn{1}{l}{\textbf{Fixed random}} & 2.25 & 3.32 & 3.53 & 1.37 \\
% \hline
\end{tabular}
\end{table}


% MB
% 4_7_22
% Fixed Random - 2249.17 & 3319.02
% Centralized - 3534.59 & 306.51
% Full information - 2920.22 & 55.53
% Greedy - 3141.58 & 618.17
% Smart EXP3 - 3530.99 & 194.25
% Smart EXP3 w/o reset - 3526.06 & 267.58
% Hybrid block EXP3 - 3486.45 & 668.62
% Block EXP3 - 3531.10 & 506.49
% EXP3 - 2889.77 & 134.14

% 11_11_11
% Fixed Random - 3534.33 & 1365.35
% Centralized - 3534.58 & 269.96
% Full information - 2704.38 & 92.53
% Greedy - 3534.67 & 599.36
% Smart EXP3 - 3618.66 & 94.18
% Smart EXP3 w/o reset - 3543.97 & 217.67
% Hybrid block EXP3 - 3551.42 & 250.01
% Block EXP3 - 3572.38 & 424.17
% EXP3 - 2731.04 & 84.31

% Fixed Random - 2249.17 & 3319.02 & 3534.33 & 1365.35 \\
% Centralized - 3534.59 & 306.51 & 3534.58 & 269.96 \\
% Full information - 2920.22 & 55.53 & 2704.38 & 92.53 \\
% Greedy - 3141.58 & 618.17 & 3534.67 & 599.36 \\
% Smart EXP3 - 3530.99 & 194.25 & 3618.66 & 94.18 \\
% Smart EXP3 w/o reset - 3526.06 & 267.58 & 3543.97 & 217.67 \\
% Hybrid block EXP3 - 3486.45 & 668.62 & 3551.42 & 250.01 \\
% Block EXP3 - 3531.10 & 506.49 & 3572.38 & 424.17 \\
% EXP3 - 2889.77 & 134.14 & 2731.04 & 84.31 \\

% GB
% Fixed Random - 2.25 & 3.32 & 3.53 & 1.37 \\
% Centralized - 3.53 & 0.31 & 3.53 & 0.27 \\
% Full information - 2.92 & 0.06 & 2.70 & 0.09 \\
% Greedy - 3.14 & 0.62 & 3.53 & 0.60 \\
% Smart EXP3 - 3.53 & 0.19 & 3.62 & 0.09 \\
% Smart EXP3 w/o reset - 3.53 & 0.27 & 3.54 & 0.22 \\
% Hybrid block EXP3 - 3.49 & 0.67 & 3.55 & 0.25 \\
% Block EXP3 - 3.53 & 0.51 & 3.57 & 0.42 \\
% EXP3 - 2.89 & 0.13 & 2.73 & 0.08 \\

% 4_7_22
% Fixed Random - 2.25 & 3.32
% Centralized - 3.53 & 0.31
% Full information - 2.92 & 0.06
% Greedy - 3.14 & 0.62
% Smart EXP3 - 3.53 & 0.19
% Smart EXP3 w/o reset - 3.53 & 0.27
% Hybrid block EXP3 - 3.49 & 0.67
% Block EXP3 - 3.53 & 0.51
% EXP3 - 2.89 & 0.13

%11_11_11
% Fixed Random - 3.53 & 1.37
% Centralized - 3.53 & 0.27
% Full information - 2.70 & 0.09
% Greedy - 3.53 & 0.60
% Smart EXP3 - 3.62 & 0.09
% Smart EXP3 w/o reset - 3.54 & 0.22
% Hybrid block EXP3 - 3.55 & 0.25
% Block EXP3 - 3.57 & 0.42
% EXP3 - 2.73 & 0.08

% Fixed Random - 2.25 & 3.32 & 3.53 & 1.37 \\
% Centralized - 3.53 & 0.31 & 3.53 & 0.27 \\
% Full information - 2.92 & 0.06 & 2.70 & 0.09 \\
% Greedy - 3.14 & 0.62 & 3.53 & 0.60 \\
% Smart EXP3 - 3.53 & 0.19 & 3.62 & 0.09 \\
% Smart EXP3 w/o reset - 3.53 & 0.27 & 3.54 & 0.22 \\
% Hybrid block EXP3 - 3.49 & 0.67 & 3.55 & 0.25 \\
% Block EXP3 - 3.53 & 0.51 & 3.57 & 0.42 \\
% EXP3 - 2.89 & 0.13 & 2.73 & 0.08 \\

% fairness
% EXP3: Jain fairness = 0.9978673463626828, min-max ratio fairness = 0.8419448307915721
% blockEXP3: Jain fairness = 0.9813642227095811, min-max ratio fairness = 0.6546272745703419
% hybridBlockEXP3: Jain fairness = 0.9684629164295961, min-max ratio fairness = 0.6201930539940086
% stableHybridBlockEXP3: Jain fairness = 0.9947163279771915, min-max ratio fairness = 0.7949326841425366
% stableHybridBlockExp3_reset: Jain fairness = 0.9971519934861299, min-max ratio fairness = 0.8299200507906908
% expWeightedAvgFullInfo: Jain fairness = 0.9996425095998146, min-max ratio fairness = 0.9307521876186523
% greedy: Jain fairness = 0.9708376092276527, min-max ratio fairness = 0.7722840795648571
% centralized: Jain fairness = 0.9932249290697854, min-max ratio fairness = 0.7855619918887092
% fixedRandom: Jain fairness = 0.6247106543125487, min-max ratio fairness = 0.18854124845942075
